AlignMiF: Geometry-Aligned Multimodal Implicit Field for LiDAR-Camera Joint Synthesis

Neural implicit fields have been a de facto standard in novel view synthesis. Recently, there exist some methods exploring fusing multiple modalities within a single field, aiming to share implicit features from different modalities to enhance reconstruction performance. However, these modalities often exhibit misaligned behaviors: optimizing for one modality, such as LiDAR, can adversely affect another, like camera performance, and vice versa. In this work, we conduct comprehensive analyses on the multimodal implicit field of LiDAR-camera joint synthesis, revealing the underlying issue lies in the misalignment of different sensors. Furthermore, we introduce AlignMiF, a geometrically aligned multimodal implicit field with two proposed modules: Geometry-Aware Alignment (GAA) and Shared Geometry Initialization (SGI). These modules effectively align the coarse geometry across different modalities, significantly enhancing the fusion process between LiDAR and camera data. Through extensive experiments across various datasets and scenes, we demonstrate the effectiveness of our approach in facilitating better interaction between LiDAR and camera modalities within a unified neural field. Specifically, our proposed AlignMiF, achieves remarkable improvement over recent implicit fusion methods (+2.01 and +3.11 image PSNR on the KITTI-360 and Waymo datasets) and consistently surpasses single modality performance (13.8% and 14.2% reduction in LiDAR Chamfer Distance on the respective datasets).

==> latex/fig/geo_fusion_feat.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{imgs/raw/geo_fusion_feat.png}
    \caption{geo-fusion feat}
    \label{fig:geo_fusion_feat}
\end{figure*}


==> latex/fig/mmnerf_feat.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{imgs/raw/mmnerf_feat.png}
    \caption{mmnerf feat}
    \label{fig:mmnerf_feat}
\end{figure*}


==> latex/fig/res_kitti_lidar.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{imgs/res_lidar.pdf}
    \caption{\textbf{Qualitative results on KITTI-360 dataset.}
    }
    \label{fig:res_kitti_lidar}
\end{figure*}


==> latex/fig/res_waymo_lidar.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{imgs/w_res_lidar.pdf}
    \caption{\textbf{Qualitative results on Waymo dataset.}
    }
    \label{fig:res_waymo_lidar}
\end{figure*}


==> latex/table/ablations.tex <==
\begin{table}[ht]
  \centering \small
  % \vspace{-0.2cm}
  \caption{\textbf{Ablation study for the proposed components.}
  }% by a comfortable margin.}
  \addtolength{\tabcolsep}{-1pt}
    \begin{tabularx}{\linewidth}{l|cc|cc}
  \toprule
 \multirow{2}{*}{Method}   & \multicolumn{2}{c|}{RGB Metric} & \multicolumn{2}{c}{LiDAR Metric}  \\
      \cmidrule(r){2-5}   & PSNR$\uparrow$ & SSIM$\uparrow$ & C-D$\downarrow$ & F-score$\uparrow$ \\
      \midrule
    i-NGP~\cite{muller2022instantNGP}& 24.45 & 0.787 &-&-\\
     LiDAR-NeRF~\cite{tao2023lidarnerf}&-&-&0.088 & 0.920\\
     % \midrule
     % \UniSim ~\cite{yang2023unisim} & 24.65 & 0.803&0.111 & 0.912\\
     \midrule
      w  \Geoinit &24.70 \plus &0.806 &0.079 \plus &0.930  \\
       % w  geo\_fusion &24.65 & & \textbf{0.156} & 0.078&0.930&0.100   \\
        w  \Geofusion &24.64 \plus& 0.810 & 0.079 \plus&0.930 \\
       % \name{}   & \textbf{24.82} &  \textbf{0.811} & 0.164 & \textbf{0.076}&\textbf{0.931}&\textbf{0.098}   \\
        \name{}   &\textbf{24.90 \plus} &\textbf{0.813}& \textbf{0.077 \plus}&\textbf{0.931}  \\


      \bottomrule
     %  \multicolumn{8}{l}{\scriptsize{M, L, C denotes modality, LiDAR, camera respectively.}}
    \end{tabularx}
  \label{tab:ablations}
\end{table}


% \begin{table}[ht]
%   \centering \small
%   % \vspace{-0.2cm}
%   \caption{\textbf{different moudule}
%   }% by a comfortable margin.}
%   \addtolength{\tabcolsep}{-5.2pt}
%     \begin{tabularx}{\linewidth}{l|ccc|ccc}
%   \toprule
%  \multirow{2}{*}{Method}   & \multicolumn{3}{c|}{RGB Metric} & \multicolumn{3}{c}{LiDAR Metric}  \\
%       \cmidrule(r){2-7}   & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & C-D$\downarrow$ & F-score$\uparrow$  & MAE$\downarrow$ \\
%       \midrule
%     i-NGP~\cite{muller2022instantNGP}& 24.45 & 0.787 &0.184 &-&-&-\\
%      LiDAR-NeRF~\cite{tao2023lidarnerf}&-&-&-&0.088 & 0.920&0.159\\
%      \midrule
%      Implicit-Fusion  & 24.65 & 0.803&0.172&0.111 & 0.912& 0.097\\
%      \midrule
%       w  geo\_init &24.70 &0.806 & 0.164 &0.079&0.930&\textbf{0.099}  \\
%        % w  geo\_fusion &24.65 & & \textbf{0.156} & 0.078&0.930&0.100   \\
%         w  geo\_fusion &24.64 & 0.810& \textbf{0.158} & 0.079&0.930&0.100 \\
%        % \name{}   & \textbf{24.82} &  \textbf{0.811} & 0.164 & \textbf{0.076}&\textbf{0.931}&\textbf{0.098}   \\
%         \name{}   &\textbf{24.90} &\textbf{0.813}& 0.161 & \textbf{0.077}&\textbf{0.931}&0.100   \\


%       \bottomrule
%      %  \multicolumn{8}{l}{\scriptsize{M, L, C denotes modality, LiDAR, camera respectively.}}
%     \end{tabularx}
%   \label{tab:ablations}
% \end{table}


==> latex/table/aiodrive_bp.tex <==

\begin{table}[ht]
  \centering \small
  % \caption{\textbf{Problem of misalignment.} When directly implicit fusing the multiple modalities cannot outperform their unimodal counterparts simultaneously in real-world datasets, e.g., KITTI-360 and Waymo. While this challenge is not present in the synthetic dataset AIODrive without misalignment issues. Here, $w$ denotes the weight ratio between the two modalities, specifically $w_\lambda = \lambda_c / \lambda_l$.}
\caption{\textbf{Problem of misalignment.} When directly implicit fusing the multiple modalities cannot outperform their unimodal counterparts simultaneously in real-world datasets. While this challenge is not present in the synthetic dataset. Here, $w$ denotes the weight ratio between the two modalities, $w_\lambda = \lambda_c / \lambda_l$.}

  \addtolength{\tabcolsep}{-3.1pt}
    \begin{tabularx}{\linewidth}{l|c|cc|cc}
  \toprule
  %
 \multirow{2}{*}{Method}   &  \multirow{2}{*}{$w_\lambda$}  & \multicolumn{2}{c|}{RGB Metric} & \multicolumn{2}{c}{LiDAR Metric}  \\
      \cmidrule(r){3-6} &   & PSNR$\uparrow$ & SSIM$\uparrow$  & C-D$\downarrow$ & F-score$\uparrow$ \\
      \midrule
       \multicolumn{3}{l}{\textit{\textbf{KITTI-360} \ts[9pt]{(real-world)}}}    \\
        \midrule

    i-NGP~\cite{muller2022instantNGP} &--& 24.45 &0.787 & --&--\\
     LiDAR-NeRF~\cite{tao2023lidarnerf} & --&--&--&0.088 & 0.920\\
      % Single Modality &--& 24.45 &0.787 & 0.088 & 0.920\\
     \midrule
        \multirow{4}{*}{\UniSim ~\cite{yang2023unisim}}
         % & 0.1& 23.64 \minus& 0.764 &0.090 \minus& 0.929 \\
         & 0.1& 23.54 \minus  &0.759  &0.087 \plus& 0.929 \\
                & 0.5& 24.38 \minus& 0.792 & 0.100 \tr[8pt]{(-) }& 0.920\\
      & 1.0 & 24.65 \plus &0.803& 0.111 \tr[8pt]{(-) }& 0.912\\
                & 2.0 &24.80 \plus & 0.809 &0.124 \minus &0.900\\
              %   & 10 &25.14 & 0.809 &0.124 &0.900\\



     \midrule
       \multicolumn{3}{l}{\textit{\textbf{Waymo} \ts[9pt]{(real-world)}}}    \\
        \midrule
     % 1319
     %     i-NGP~\cite{muller2022instantNGP} &--& 28.45 &0.854 & --&--\\
     % LiDAR-NeRF~\cite{tao2023lidarnerf} & --&--&--&0.101 & 0.922\\
     % \midrule
     %   \multirow{4}{*}{\UniSim ~\cite{yang2023unisim}}
     %            & 0.5& 26.74 \minus & 0.817 & 0.096 \plus & 0.929\\
     %  & 1.0 & 27.82 \minus &0.839& 0.108 \minus & 0.920\\
     % & 2.0 & 28.24 \minus &0.849& 0.130 \minus & 0.905\\
     %            & 5.0 &28.51 \plus & 0.855 &0.150 \minus & 0.882\\
    % 1776
    i-NGP~\cite{muller2022instantNGP} &--& 28.20 &0.830 & --&--\\
     LiDAR-NeRF~\cite{tao2023lidarnerf} & --&--&--&0.179 & 0.885\\
     %   Single Modality &--& 28.20 &0.830 &0.179 & 0.885\\
     \midrule
       \multirow{4}{*}{\UniSim ~\cite{yang2023unisim}}
                & 0.5& 26.41 \minus & 0.789 & 0.172 \plus & 0.891\\
    & 1.0 & 27.12 \minus &0.805& 0.181 \minus & 0.885\\
      & 2.0 & 27.72 \minus& 0.818 & 0.200 \minus &0.865\\
                & 5.0 &28.33 \plus & 0.830 &0.227 \minus & 0.840\\

    \midrule
       \multicolumn{3}{l}{\textit{\textbf{AIODrive} \ts[9pt]{(synthetic)}}}    \\
        \midrule
         i-NGP~\cite{muller2022instantNGP} &--& 34.43 &0.893 & --&--\\
     LiDAR-NeRF~\cite{tao2023lidarnerf} & --&--&--&0.178 & 0.873\\
    % Single Modality   &--& 34.43 &0.893 &0.178 & 0.873\\
     \midrule
       \multirow{3}{*}{\UniSim ~\cite{yang2023unisim}}
       & 0.1& 34.25  \minus &  0.901 & 0.138 \plus& 0.921\\
           % & 0.5& 34.35  \minus &  0.902 & 0.139 \plus& 0.915\\
                % & 0.5& 34.18  \minus &  0.899 & 0.136 \plus& 0.919\\
      & 1.0 &  \CC 34.53 \plus & \CC 0.904 & \CC 0.153 \plus & \CC 0.915\\
                & 5.0 &34.64 \plus & 0.905 &0.191 \minus &0.914\\

      \bottomrule
    \end{tabularx}
  \label{tab:aiodrive}
\end{table}
\vspace{-6pt}


==> latex/table/all_res_bp.tex <==
\begin{table*}[ht]
  \centering
  \small
  % \footnotesize
  % \vspace{-0.2cm}
  \caption{\textbf{Novel view synthesis on KITTI-360 dataset and Waymo dataset}. \name{} outperforms the baseline in all metrics.
  }% by a comfortable margin.}
  \addtolength{\tabcolsep}{-4.4pt}
    \begin{tabularx}{0.95\linewidth}{l|c|ccc|ccc||ccc|ccc}
  \toprule
 \multirow{3}{*}{Method} &
 \multirow{3}{*}{M}  & \multicolumn{6}{c||}{KITTI-360 Dataset} & \multicolumn{6}{c}{Waymo Dataset}  \\
 \cmidrule(r){3-14} & & \multicolumn{3}{c|}{RGB Metric} & \multicolumn{3}{c||}{LiDAR Metric} & \multicolumn{3}{c|}{RGB Metric} & \multicolumn{3}{c}{LiDAR Metric} \\
       &    & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & C-D$\downarrow$ & F-score$\uparrow$  & MAE$\downarrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & C-D$\downarrow$ & F-score$\uparrow$  & MAE$\downarrow$\\
      \midrule


   \multicolumn{2}{l|}{Sequence} & \multicolumn{6}{l||}{\textit{Seq 1538--1601 }} & \multicolumn{6}{l}{\textit{seg11379226583756500423\_6230\_810\_6250\_810}} \\
       \midrule
    i-NGP~\cite{muller2022instantNGP}&C & 25.22 & 0.831 & 0.175 & --&--&-- &29.26 &0.825& 0.369 & --&--&--\\
     LiDAR-NeRF~\cite{tao2023lidarnerf}&L & --&--&-- & 0.085 &0.925&0.107 & --&--&-- & 0.216 & 0.853 &0.026\\
     \UniSim ~\cite{yang2023unisim} &LC & 22.92 \minus  &0.746 & 0.328 &0.083 \plus& 0.927 &0.103 &
     26.90 \minus  & 0.777& 0.399 &0.199 \plus &0.854 &0.027
     \\
     \UniSim ~\cite{yang2023unisim} &LC & 25.25 \plus & 0.827& 0.184 &0.109 \minus &0.904 &0.102 &
     29.35 \plus &0.825& 0.367 &0.359 \minus & 0.761 &0.030
     \\
    \LC   \name{}  &LC & 25.31 \plus &0.836  &0.169  &0.077 \plus &0.926  &0.107 & 29.92 \plus &0.833& 0.347& 0.197 \plus& 0.859 &0.026\\

     \midrule
   \multicolumn{2}{l|}{Sequence} & \multicolumn{6}{l||}{\textit{Seq 1728--1791 }} & \multicolumn{6}{l}{\textit{seg10676267326664322837\_311\_180\_331\_180}} \\
       \midrule
    i-NGP~\cite{muller2022instantNGP}&C & 24.90 & 0.816 & 0.167  & --&--&-- & 29.52 &0.861 &0.299 & --&--&-- \\
     LiDAR-NeRF~\cite{tao2023lidarnerf}&L & --&--&--&0.107 & 0.895& 0.111 & --&--&--&   0.264 &0.841 &0.026\\
     \UniSim ~\cite{yang2023unisim} &LC & 23.86 \minus  & 0.782 & 0.228 & 0.097 \plus&  0.909 & 0.094 &
     26.47 \minus  & 0.808  & 0.341  & 0.254 \plus  & 0.848  & 0.026
     \\
     \UniSim ~\cite{yang2023unisim} &LC &25.38 \plus &0.823& 0.167 &0.127 \minus& 0.891 &0.093 &
     29.56 \plus & 0.862 &0.299 &1.006 \minus &0.584 &0.037

     \\
    \LC   \name{}  &LC &25.29 \plus& 0.831 &0.146 &0.087 \plus& 0.913& 0.096& 29.82 \plus &0.867 &0.285 &0.243 \plus &0.850 &0.025\\

    \midrule
   \multicolumn{2}{l|}{Sequence} & \multicolumn{6}{l||}{\textit{Seq 1908--1971 }} & \multicolumn{6}{l}{\textit{seg17761959194352517553\_5448\_420\_5468\_420}} \\
       \midrule
  % i-NGP~\cite{muller2022instantNGP}&C & 24.47 & 0.788 & 0.183 &-&-&-\\
  %    LiDAR-NeRF~\cite{tao2023lidarnerf}&L &-&-&-&0.083 & 0.932&0.100\\
  %    \UniSim ~\cite{yang2023unisim} &LC & 24.69 &0.802&0.172&0.115 & 0.913&0.098\\
  %    \name{}  &LC &24.90 &0.813& 0.161 & 0.077&0.931&0.100   \\
      i-NGP~\cite{muller2022instantNGP}&C & 24.45 &0.787 &0.184 & --&--&-- & 28.20 &  0.830 & 0.372 & --&--&--\\
     LiDAR-NeRF~\cite{tao2023lidarnerf}&L & --&--&--&0.088 & 0.920&0.159 &--&--&--& 0.179& 0.885 &0.049\\
     \UniSim ~\cite{yang2023unisim} &LC & 23.54 \minus  &0.759 & 0.235 &0.087 \plus& 0.929 & 0.097 & 26.41 \minus & 0.789& 0.403 &0.173 \plus& 0.891 &0.049\\
     \UniSim ~\cite{yang2023unisim} &LC & 24.65 \plus& 0.803 &0.172&0.111 \minus& 0.912&0.097& 28.33 \plus &0.830 &0.369 &0.227 \minus &0.840 & 0.052\\
      % \name{}  &LC &24.82 & 0.811 & 0.164 & 0.076&0.931&0.098   \\
    \LC   \name{}  &LC &24.90 \plus&0.813& 0.161 & 0.077 \plus&0.931&0.100   & 28.78 \plus & 0.835 & 0.347& 0.152 \plus& 0.892 &0.047\\


          \midrule
   \multicolumn{2}{l|}{Sequence} & \multicolumn{6}{l||}{\textit{Seq 3353--3416 }} & \multicolumn{6}{l}{\textit{seg1172406780360799916\_1660\_000\_1680\_000}} \\
       \midrule
    i-NGP~\cite{muller2022instantNGP}&C & 23.88 & 0.800& 0.199 & --&--&-- &28.30 &0.810 &0.480 & --&--&--\\
     LiDAR-NeRF~\cite{tao2023lidarnerf}&L & --&--&--& 0.094 &0.927 &0.112& --&--&-- &0.127 &0.908 &0.057\\
     \UniSim ~\cite{yang2023unisim} &LC & 22.90 \minus  & 0.746& 0.283 &0.091 \plus& 0.933 & 0.093\\
     \UniSim ~\cite{yang2023unisim} &LC &24.51 \plus &0.797& 0.213  &0.110 \minus&0.919& 0.091 &
     28.72 \plus& 0.816& 0.463& 0.225 \minus &0.841 &0.058\\
    \LC   \name{}  &LC & 24.74 \plus & 0.810 &0.182& 0.086 \plus & 0.937& 0.096
    & 28.84 \plus &0.819& 0.449 &0.107 \plus & 0.918& 0.054\\


            \midrule
   \multicolumn{8}{l}{Average } & \multicolumn{6}{l}{Average }\\
       \midrule
    i-NGP~\cite{muller2022instantNGP}&C & 24.61 & 0.808 & 0.181 & --&--&-- \\
     LiDAR-NeRF~\cite{tao2023lidarnerf}&L & --&--&--& 0.093 & 0.916 & 0.122 \\
     \UniSim ~\cite{yang2023unisim} &LC & 23.30 \minus  & 0.758 & 0.268 & 0.090 \plus& 0.924 & 0.097\\
     \UniSim ~\cite{yang2023unisim} &LC & 24.94 \plus&	0.812&	0.184&	0.114 \minus&0.906&	0.095\\
   \LC   \name{}  &LC & 25.06 \plus&	0.823	&0.165&	0.081 \plus&	0.927	&0.099\\



      \bottomrule
      \multicolumn{8}{l}{\scriptsize{M, L, C denotes modality, LiDAR, camera respectively.}}
    \end{tabularx}
  \label{tab:all_res_bp}
\end{table*}


==> latex/table/load_lidar.tex <==

\begin{table}[ht]
  \centering \small
  % \vspace{-0.2cm}
  \caption{\textbf{Ablation study for the design of the proposed components.}}
  \addtolength{\tabcolsep}{-1pt}
    \begin{tabularx}{\linewidth}{l|cc|cc}
  \toprule
 \multirow{2}{*}{Method}   & \multicolumn{2}{c|}{RGB Metric} & \multicolumn{2}{c}{LiDAR Metric}  \\
      \cmidrule(r){2-5} & PSNR$\uparrow$ & SSIM$\uparrow$  & C-D$\downarrow$ & F-score$\uparrow$ \\
      \midrule
    i-NGP~\cite{muller2022instantNGP}& 24.45 &0.787 & --&--\\
     LiDAR-NeRF~\cite{tao2023lidarnerf} & --&--&0.088 & 0.920\\


     \midrule
        \multicolumn{3}{l}{\textit{\textbf{\Geoinit}}}    \\
        \midrule

     Load LiDAR encoder & 24.34& 0.784 & 0.096 & 0.920  \\
     + Fix LiDAR encoder  & 18.60 & 0.537 & 0.120 & 0.904  \\
     Detach RGB Density & 12.41 & 0.597 & 0.098 & 0.916  \\


     \midrule
        \multicolumn{3}{l}{\textit{\textbf{\Geofusion}}}    \\
        \midrule

        Addition& 24.47 &0.808 & 0.081& 0.929 \\
        Attention& 24.48&  0.791&  0.089 &0.929\\
        Concatenation & 24.64 & 0.810 & 0.079&0.930\\


      \bottomrule
     %  \multicolumn{4}{l}{\scriptsize{M, L, C denotes modality, LiDAR, camera respectively.}}
    \end{tabularx}
  \label{tab:load_lidar}
\end{table}


==> latex/table/model_size.tex <==

\begin{table}[ht]
  \centering \small
  % \vspace{-0.2cm}
  \caption{\textbf{sota on synthetic dataset } 13.62M }
  \addtolength{\tabcolsep}{-2.8pt}
    \begin{tabularx}{\linewidth}{l|ccc}
  \toprule
  %
 Method & Model-size & Training-time & Performance  \\
    \midrule
      \UniSim ~\cite{yang2023unisim} & 13.65M & 1.23 hours &    24.38 \ 0.100 \\
        %  w/  \Geoinit & 27.26992 & & 24.70 \ 0.079  \\
        % w/  \Geofusion &  27.26992 & & 24.64 \ 0.079   \\
        \name{} & 27.26M & 2.55 hours & 25.20 \ 0.077   \\

      \bottomrule
    \end{tabularx}
  \label{tab:model_size}
\end{table}

